Exploring User Privacy Awareness on GitHub: An Empirical Study

GitHub provides developers with a practical way to distribute source code and collaboratively work on common projects. To enhance account security and privacy, GitHub allows its users to manage access permissions, review audit logs, and enable two-factor authentication. However, despite the endless effort, the platform still faces various issues related to the privacy of its users. This paper presents an empirical study delving into the GitHub ecosystem. Our focus is on investigating the utilization of privacy settings on the platform and identifying various types of sensitive information disclosed by users. Leveraging a dataset comprising 6,132 developers, we report and analyze their activities by means of comments on pull requests. Our findings indicate an active engagement by users with the available privacy settings on GitHub. Notably, we observe the disclosure of different forms of private information within pull request comments. This observation has prompted our exploration into sensitivity detection using a large language model and BERT, to pave the way for a personalized privacy assistant. Our work provides insights into the utilization of existing privacy protection tools, such as privacy settings, along with their inherent limitations. Essentially, we aim to advance research in this field by providing both the motivation for creating such privacy protection tools and a proposed methodology for personalizing them.

==> commands.tex <==

% Usual suspects
\usepackage{xspace}
\usepackage{amssymb}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{xcolor}
\newcommand{\nb}[2]{
	\fbox{\bfseries\sffamily\scriptsize#1}
	{\sf$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
}

\newcommand*{\ie}{i.e.,\@\xspace}
\newcommand*{\eg}{e.g.,\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}

\newcommand*{\RM}{README\@\xspace}
\newcommand*{\SR}{SOrec\@\xspace}
\newcommand*{\SO}{StackOverflow\@\xspace}
\newcommand*{\GH}{GitHub\@\xspace}
\newcommand*{\PR}{PROMPTER\@\xspace}
\newcommand*{\CS}{CrossSim\@\xspace}
\newcommand*{\CR}{CrossRec\@\xspace}
\newcommand*{\FC}{FOCUS\@\xspace}
\newcommand*{\AU}{AURORA\@\xspace}
\newcommand*{\FaC}{FaCoY\@\xspace}


\newcommand*{\CM}{CROSSMINER\@\xspace}
\newcommand*{\LP}{LUPE\@\xspace}
\newcommand*{\NM}{NEMO\@\xspace}
\newcommand*{\DL}{DeepLib\@\xspace}
\newcommand*{\EP}{EvoPlan\@\xspace}
\newcommand*{\GS}{GitSum\@\xspace}
\newcommand*{\PL}{PILOT\@\xspace}
\newcommand*{\MG}{MORGAN\@\xspace}
\newcommand*{\CB}{CodeBERT\@\xspace}
\newcommand*{\TF}{T5\@\xspace}


\makeatletter
\newcommand*{\etc}{%
	\@ifnextchar{.}%
	{etc}%
	{etc.\@\xspace}%
}
\makeatother
%\newcommand*{\etal}{\emph{et~al.}\@\xspace}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

%\newcommand{\nb}[2]{\fbox{\bfseries\sffamily\scriptsize#1}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}
%\newcommand{\nb}[2]{\fbox{\bfseries\sffamily\scriptsize#1} {\sf\small 
%\textit{#2} }}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\color{black} 
		\node[shape=circle,draw=cyan,fill=black!10!white,inner sep=.3pt] (char) 
		{{{\texttt\textbf #1}}};}}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) 
-- cycle;} 

\newcommand\CA[1]{\textcolor{green}{\nb{Costanza}{#1}}}

\newcommand\JDR[1]{\textcolor{purple}{\nb{Juri} {#1}}}

\newcommand\PN[1]{\textcolor{red}{\nb{Phuong}{#1}}}


\newcommand\revised[1]{\textcolor{blue}{#1}}

\newcommand{\code}[1]{{\texttt{#1}}}

\newcommand{\projectName}{CROSSMINER\@\xspace}
\newcommand{\CrossSim}{CrossSim\@\xspace}
\newcommand{\CrossRec}{CrossRec\@\xspace}
\newcommand{\bnetwork}{MNBN}
\newcommand{\focus}{FOCUS\@\xspace}
\newcommand{\sorec}{SOrec\@\xspace}


\newcommand*{\rs}{recommendation systems\@\xspace} 


\newcommand{\challenge}[2]{
	\begin{tcolorbox}[boxrule=0.5pt]
		{\bfseries #1}: {#2}
	\end{tcolorbox}
}

\definecolor{darkgray}{gray}{0.78}
\definecolor{lightgray}{gray}{0.85}
\definecolor{verylightgray}{gray}{0.95}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}




\newcommand*{\numDevs}{6,132\@\xspace}
%
%\lstset{numbers=left,
%	inputencoding=latin1,
%	basicstyle=\footnotesize\ttfamily,
%	keywordstyle=\color{blue},         
%	breaklines=true, 
%	showtabs=false,
%	showstringspaces=false,
%	numberstyle=\tiny\color{gray}
%}



%Code listing style named "mystyle"
\lstdefinestyle{java}{
	backgroundcolor=\color{backcolour},   commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\ttfamily\scriptsize,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	numbersep=5pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

%"mystyle" code listing set
\lstset{style=java}

==> tex/tables.tex <==




\begin{comment}
STEP - SOURCE - #USERS - #PR COMMENTS - #COMMIT COMMENTS  - #Issues comments
_______________________________________________________________
STEP 1 GHTorrent - 30.456.000 da
STEP 2 Active users - 6400  3123    1231123
STEP 3 GH API actualization - 54545 - 12312312 
\end{comment}



\begin{table}[H]
\footnotesize
\begin{tabular}{cp{1cm}p{1cm}p{1cm}p{1cm}p{1.3cm}}
\toprule
\textbf{Step} & \textbf{Source} & \textbf{\#Users} & \textbf{Final \#Users } &\textbf{\#Pr Comments} & \textbf{\#Commit Comments} \\
\midrule
Step 1 & GHTorrent \textit{Users} & 32,411,628 & 22,525,012 & pr COMM & c COMM \\
\hfill
Step 2 & \textit{Active users} & 6,329 & 6,132 & pr COMM & c COMM \\
\hfill
Step 3 & \GH API actualization &   &   &    &    \\
\bottomrule
\end{tabular}
\caption{Data curation process}
\label{tab:userpre}
\end{table}


&           1.2e+05 &         1.2e+05 &       1.2e+05 &               1.2e+05 &              1.2e+05 \\\\\nmean  &           4.9e-04 &         1.5e-03 &       3.9e-03 &               2.5e-03 &              4.9e-03 \\\\\nstd   &           4.4e-03 &         9.7e-03 &       1.2e-02 &               1.2e-02 &              1.5e-02 \\\\\nmin   &           0.0e+00 &         0.0e+00 &       0.0e+00 &               0.0e+00 &              0.0e+00 \\\\\n50\\%   &           0.0e+00 &         3.7e-04 &       7.1e-04 &               5.1e-04 &              1.0e-03 \\\\\n65\\%   &           3.3e-05 &         6.1e-04 &       1.8e-03 &               1.0e-03 &              2.1e-03 \\\\\n75\\%   &           9.8e-05 &         9.3e-04 &       3.3e-03 &               1.7e-03 &              3.5e-03 \\\\\nmax   &           1.0e+00 &         1.0e+00 &       1.0e+00 &               1.0e+00 &              1.0e+00 \\\\\n\\bottomrule\n\\end{tabular}\n'

==> tex/threatstovalidity.tex <==
\begin{enumerate}
    \item GhTorrent from 2019 \CA{write first and then we classify}
    \item Only comments from PR comments and not other types of comments: nelle pullrequest esprimono più pareri/discussions 
    \item Active users are active according to the GHTorrent from 2019 (indeed, while updating, we dropped some users that no longer existed in GitHub)
    \item what users express in their settings might not correspond to their privacy desiderata therefore the conclusions of the privacy paradox are not so solid
\end{enumerate}
